Can LLMs Configure Software Tools

In software engineering, the meticulous configuration of software tools is crucial in ensuring optimal performance within intricate systems. However, the complexity inherent in selecting optimal configurations is exacerbated by the high-dimensional search spaces presented in modern applications. Conventional trial-and-error or intuition-driven methods are both inefficient and error-prone, impeding scalability and reproducibility. In this study, we embark on an exploration of leveraging Large-Language Models (LLMs) to streamline the software configuration process. We identify that the task of hyperparameter configuration for machine learning components within intelligent applications is particularly challenging due to the extensive search space and performance-critical nature. Existing methods, including Bayesian optimization, have limitations regarding initial setup, computational cost, and convergence efficiency. Our work presents a novel approach that employs LLMs, such as Chat-GPT, to identify starting conditions and narrow down the search space, improving configuration efficiency. We conducted a series of experiments to investigate the variability of LLM-generated responses, uncovering intriguing findings such as potential response caching and consistent behavior based on domain-specific keywords. Furthermore, our results from hyperparameter optimization experiments reveal the potential of LLMs in expediting initialization processes and optimizing configurations. While our initial insights are promising, they also indicate the need for further in-depth investigations and experiments in this domain.

==> sections/motivation.tex <==
% \textbf{\textit{RQ1: Are LLM's useful to configure software tools ?}}

% \textbf{RQ1.1: \textit{What is the inherent variability of weights within a given scenario?}}

% \textbf{RQ1.2: \textit{What is the variability of weights across different scenarios?}}

Software configuration, particularly hyperparameter optimization, is a complex and laborious task. Consider the case of Tom, an experienced programmer, who finds himself constantly wrestling with this challenge \cite{wu2019hyperparameter}. 
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/Motivation.png}
    \caption{Wu et.al,2019 research showing the number of iterations to find the right hyperparameters for improving the prediction accuracy of a model proposed in \cite{Krizhevsky2010} on CIFAR-10 dataset}
    \label{fig:motivation}
\end{figure}
Each new project he embarks on requires a meticulous, painstaking process of tuning hyperparameters to optimize software performance. The expansive configuration space and interdependencies among various parameters makes this a daunting task \cite{belete2022grid, victoria2021automatic}. Tom often finds himself caught in an iterative cycle of tweaking and testing, making incremental adjustments based on a combination of past experiences, expert insights, and sheer trial and error.

Furthermore, the time and effort Tom expends on this process are substantial. Each iteration requires careful selection, adjustment, and evaluation of configuration parameters This time-intensive, manual effort not only hinders the software's time-to-market but also increases project overheads \cite{eimer2023hyperparameters, luketina2016scalable}, making the configuration process an expensive endeavour \cite{wu2019hyperparameter}. 
The high dimensionality and complexity of the configuration space means that even a minor oversight can have significant implications on software performance. Any mistake or incorrect choice can lead to sub-optimal performance, causing Tom to go back to the drawing board, thereby elongating the development cycle \cite{luketina2016scalable}.

